Optimizing Fiducial Marker Placement for Improved Visual Localization

Adding fiducial markers to a scene is a well-known strategy for making visual localization algorithms more robust. Traditionally, these marker locations are selected by humans who are familiar with visual localization techniques. This paper explores the problem of automatic marker placement within a scene. Specifically, given a predetermined set of markers and a scene model, we compute optimized marker positions within the scene that can improve accuracy in visual localization. Our main contribution is a novel framework for modeling camera localizability that incorporates both natural scene features and artificial fiducial markers added to the scene. We present optimized marker placement (OMP), a greedy algorithm that is based on the camera localizability framework. We have also designed a simulation framework for testing marker placement algorithms on 3D models and images generated from synthetic scenes. We have evaluated OMP within this testbed and demonstrate an improvement in the localization rate by up to 20 percent on four different scenes.

==> introduction.tex <==
\section{Introduction}
Visual localization is a foundational technique for applications including AR/VR, autonomous driving, and robotic navigation and manipulation. A typical problem in visual localization is to estimate the camera pose of a query image, provided a pre-built map. While the problem has long been investigated in many fields~\cite{zhang2021reference}, visual localization still suffers due to challenging scenes such as textureless walls and repetitive structures (e.g., Rooms A and B in Fig.~\ref{fig:demo-challenges}). One common solution to these challenges is to place fiducial markers as additional texture and identifiers in the scene~\cite{munoz2020ucoslam,DeGol_2018_ECCV}; however, placing fiducial markers in larger environments is a time consuming process and the resulting performance improvement depends on marker positions. Thus, optimizing marker placement is valuable for robust visual localization.

This work proposes an automatic approach to optimizing marker placement such that 1) the resulting marker positions yield improved accuracy in visual localization and 2) a human user will be able to place markers at positions planned by the approach (e.g., no markers on the ceiling). Specifically, the approach computes optimized marker positions, given a predetermined set of markers and a scene model. The key contributions of this work include:
\begin{enumerate}
    \item This is the first work that optimizes marker placement for visual localization based on scene features and fiducial markers.
    \item We propose a novel framework that models localizability of camera poses in a scene and computes localizability scores.
    \item We develop a greedy algorithm that optimizes marker positions with the goal of increased localizability scores.
    \item We design a simulation framework for testing marker placement algorithms on 3D scene models that enables others to reproduce and build on our work.
    \item We demonstrate that optimized marker placement by our approach can improve the localization rate by up to 20 percent on four different scenes.
\end{enumerate}

\begin{figure}[!t]
    \centering
    \includegraphics[width=.9\linewidth]{figs/showcase_hard.pdf}
    \caption{Three challenging examples for visual localization within the same scene. The images on the left and middle show two almost identical rooms in the scene, whereas the image on the right depicts a very weakly textured surface. Marker placements\protect\footnotemark in this scene guided by our optimized marker placement approach led to improved visual localization on these examples.
    }
    \label{fig:demo-challenges}
\end{figure}
\footnotetext{Fiducial markers in the examples are AprilTags\cite{olson2011apriltag} but our algorithm is general and can be used with any existing family of fiducial markers.}

%\subsection*{Notation}
%Deterministic values are denoted by lowercase letters while random variables are indicated by uppercase letters. A set of values is denoted by calligraphic font (e.g., $\mathcal{L}=\{l\}$). We use $p(X)$ to denote the probability density function $p_X(\boldsymbol{\cdot})$ of random variable $X$.
